Colliding Winds in Low-Mass Binary Star Systems: wind interactions and implications for habitable planets

Context. In binary star systems, the winds from the two components impact each other, leading to strong shocks and regions of enhanced density and temperature. Potentially habitable circumbinary planets must continually be exposed to these interactions regions. Aims. We study, for the first time, the interactions between winds from low-mass stars in a binary system, to show the wind conditions seen by potentially habitable circumbinary planets. Methods. We use the advanced 3D numerical hydrodynamic code Nurgush to model the wind interactions of two identical winds from two solar mass stars with circular orbits and a binary separation of 0.5 AU. As input into this model, we use a 1D hydrodynamic simulation of the solar wind, run using the Versatile Advection Code. We derive the locations of stable and habitable orbits in this system to explore what wind conditions potentially habitable planets will be exposed to during their orbits. Results. Our wind interaction simulations result in the formation of two strong shock waves separated by a region of enhanced density and temperature. The wind-wind interaction region has a spiral shape due to Coriolis forces generated by the orbital motions of the two stars. The stable and habitable zone in this system extends from approximately 1.4 AU to 2.4 AU. (TRUNCATED)

==> Journals.tex <==
\newcommand{\aj}{{AJ}}			
\newcommand{\araa}{{Ann.\ Rev.\ Astron.\ Astrophys.}}		
\newcommand{\apj}{{ApJ}}			
\newcommand{\apjl}{{ApJ Lett.}}		
\newcommand{\apjs}{{ApJS}}		
\newcommand{\apss}{{Ap\&SS}}		
\newcommand{\aap}{{A\&A.}}		
\newcommand{\aapr}{{A\&A~Rev.}}		
\newcommand{\aaps}{{A\&AS}}		
\newcommand{\an}{{AN}}			
\newcommand{\azh}{{AZh}}			
\newcommand{\baas}{{BAAS}}		
\newcommand{\BAIC}{{Bull.\ Astron.\ Inst.\ Czech.}}		
\newcommand{\jrasc}{{JRASC}}		
\newcommand{\memras}{{MmRAS}}		
\newcommand{\mnras}{{MNRAS}}		
\newcommand{\pra}{{Phys.~Rev.~A}}	
\newcommand{\prb}{{Phys.~Rev.~B}}	
\newcommand{\prc}{{Phys.~Rev.~C}}	
\newcommand{\prd}{{Phys.~Rev.~D}}	
\newcommand{\pre}{{Phys.~Rev.~E}}	
\newcommand{\prl}{{Phys.~Rev.~Lett.}}	
\newcommand{\pasp}{{PASP}}		
\newcommand{\pasj}{{PASJ}}		
\newcommand{\qjras}{{QJRAS}}		
\newcommand{\skytel}{{S\&T}}		
\newcommand{\solphys}{{Solar~Phys.}}	
\newcommand{\sovast}{{Soviet~Ast.}}	
\newcommand{\ssr}{{Space~Sci.~Rev.}}	
\newcommand{\zap}{{ZAp}}			
\newcommand{\nat}{{Nature}}		
\newcommand{\iaucirc}{{IAU~Circ.}}
\newcommand{\aplett}{{Astrophys.~Lett.}}
\newcommand{\apspr}{{Astrophys.~Space~Phys.~Res.}}
\newcommand{\bain}{{Bull.~Astron.~Inst.~Netherlands}}
\newcommand{\fcp}{{Fund.~Cosmic~Phys.}}
\newcommand{\gca}{{Geochim.~Cosmochim.~Acta}}
\newcommand{\grl}{{Geophys.~Res.~Lett.}}
\newcommand{\GAFD}{{Geophys.~Astrophys.~Fluid~Dyn.}}
\newcommand{\jcp}{{J.~Chem.~Phys.}}	
\newcommand{\jgr}{{J.~Geophys.~Res.}}	
\newcommand{\jqsrt}{{J.~Quant.~Spec.~Radiat.~Transf.}}
\newcommand{\memsai}{{Mem.~Soc.~Astron.~Italiana}}
\newcommand{\nphysa}{{Nucl.~Phys.~A}}
\newcommand{\physrep}{{Phys.~Rep.}}
\newcommand{\physscr}{{Phys.~Scr}}
\newcommand{\planss}{{Planet.~Space~Sci.}}
\newcommand{\procspie}{{Proc.~SPIE}}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
